SynthesizRR: Generating Diverse Datasets with Retrieval Augmentation

It is often desirable to distill the capabilities of large language models (LLMs) into smaller student models due to compute and memory constraints. One way to do this for classification tasks is via dataset synthesis, which can be accomplished by generating examples of each label from the LLM. Prior approaches to synthesis use few-shot prompting, which relies on the LLM's parametric knowledge to generate usable examples. However, this leads to issues of repetition, bias towards popular entities, and stylistic differences from human text. In this work, we propose Synthesize by Retrieval and Refinement (SynthesizRR), which uses retrieval augmentation to introduce variety into the dataset synthesis process: as retrieved passages vary, the LLM is seeded with different content to generate its examples. We empirically study the synthesis of six datasets, covering topic classification, sentiment analysis, tone detection, and humor, requiring complex synthesis strategies. We find that SynthesizRR greatly improves lexical and semantic diversity, similarity to human-written text, and distillation performance, when compared to 32-shot prompting and four prior approaches. We release our code to perform all steps at https://github.com/amazon-science/synthesizrr

==> appendices/baselines-description.tex <==
Here, we explore how \ours{} directly compares to prior work on synthesis of popular datasets. We compare against six prior approaches: 

\insection[]{\ZeroGen{} \cite{Ye2022ZeroGenEZ}:} a simple approach which uses zero-shot generation from \GPTTwoXL{} under different prompting schemes. For certain tasks like \IMDb{} and \SST, the authors occasionally seed the prompt with a previously-generated movie name (described subsequently).

% \insection[]{\ProGen{} \cite{ye-etal-2022-progen}:} generates a small synthetic dataset, then uses a student model along with an influence function to highlight high-quality generations. These are used as in-context examples for another round of generation.

\insection[]{\SunGen{} \cite{gao2023selfguided}:} uses the \ZeroGen{} strategy to generate a large synthetic dataset (200k rows). Then, uses a custom bi-level optimization algorithm (involving the student model) to determine instance-weights of each synthetic example. 

\insection[]{\ReGen{} \cite{yu-etal-2023-regen}:} performs multi-round filtering of retrieved results using 2 BERT models; one trained for retrieval, and one classifier. Use consistency between these models to filter noisy data. 

\insection[]{\LetsSynth{} \cite{wang-etal-2023-lets}:} Constructs a ``seed dataset'' (different from ours) and trains a student model. Then, extrapolate errors using an LLM and synthesizes additional data. We combine this with the seed data and repeat the process.

\insection[]{\AttrPrompt{} \cite{yu2023large}:} a method focused on improving diversity and unbiasedness of generated datasets. Prompts a powerful LLM like \ChatGPT{} with different attributes, each along different dimensions. Attributes are extracted from a human-in-the-loop analysis of task using \ChatGPT{}.

We note that zero shot generation and few-shot generation has already been compared in \autoref{tab:student-deb}, so we do not include it here.

We benchmark four classification tasks which are popular in prior work: \YelpPolarity{} \citep{zhang2015character}, \IMDb{} \cite{maas-etal-2011-learning}, \SST{} \cite{socher-etal-2013-recursive} and \AGNews{} \citep{zhang2015character}. The first three tasks are binary sentiment analysis, whereas the last is multi-class topic classification.

For the content sourcing stage of \ours, we retrieve documents from the following corpora:
\begin{itemize}
\item \YelpPolarity: to generate positive and negative reviews about businesses, we retrieve from the \YelpDataset{} corpus \cite{yelpcorpus} which contains details of 150k businesses. Each document contains the the name, address, and various tags and boolean attributes for a single business.
\item \IMDb{} and \SST: to generate movie reviews, we retrieve from the \CMUMovies{} corpus \cite{bamman-etal-2013-learning}, which contains 42k plot summaries. Each document is a plot summary for a single movie.
\item \AGNews: we use \RealNewsDominant{} from \autoref{tab:corpus}.
\end{itemize}

We note that the \CMUMovies{} and \YelpDataset{} corpora are between one to three orders of magnitude smaller than corpora in \autoref{tab:corpus}, thus it helps us evaluate \ours{} with smaller corpora. We include two different retrieval approaches: \Contriever{} (semantic match) and \BM{} (lexical match).

Following \citet{yu2023large}, we generate 6,000 rows using the \ours{} \RetrICL{} variant described in Algorithm~\ref{alg:synthesizrr}. We generate an equal number of examples for each class. We calculate intrinsic metrics Self-BLEU-5, MAUVE and Entity Entropy as described in \S\ref{sec:expt-setup}. 

Prior work often generates much larger datasets (20k to 200k examples) and uses different student model hyperparameters. Intrinsic evaluations of dataset quality are also seldom reported. This makes it difficult to fairly compare results from previous papers. Thus, we reproduce results ourselves by using synthetic datasets released by the authors, after subsampling to 6,000 examples. We report distillation results in \autoref{tab:baselines-student} and intrinsic metrics in \autoref{tab:baselines-intrinsic}.

==> table/baselines-combined-main.tex <==
\begin{table}[!t]
\centering
\sisetup{round-mode=places, round-precision=1} % Set the rounding precision
\setlength{\tabcolsep}{1.9pt}
\footnotesize{

\begin{tabular}{
C{1.1cm}  % Method
h % C{1.15cm}  % Retriever
C{1.2cm}  % Teacher LLM
% h % c % S[table-format=3.2]  % Yelp Self-BLEU
% c % S[table-format=3.2]  % AG News Self-BLEU
% C{0.7cm} % S[table-format=3.2]  % IMDb Self-BLEU
% c % S[table-format=3.2]  % SST-2 Self-BLEU
% c 
% h %|c % S[table-format=3.2]  % Yelp Entity Entropy
% |c % S[table-format=3.2]  % AG News Entity Entropy
% C{0.7cm} % S[table-format=3.2]  % IMDb Entity Entropy
% c  % S[table-format=3.2]  % SST-2 Entity Entropy
% c 
h %|c % S[table-format=3.2]  % Yelp Mauve
C{0.55cm} % S[table-format=3.2]  % AG News Mauve
C{0.75cm} % S[table-format=3.2]  % IMDb Mauve
c % S[table-format=3.2]  % SST-2 Mauve
% c 
h %|c % S[table-format=3.2]  % Yelp Accuracy
|C{0.6cm} % S[table-format=3.2]  % AG News Accuracy
C{0.75cm} % S[table-format=3.2]  % IMDb Accuracy
c % S[table-format=3.2]  % SST-2 Accuracy
}
\toprule
% \multirow{3}{*}{\textbf{Method}}
% & \multirow{3}{*}{ \textbf{Student LM} }
% & \multicolumn{1}{c}{\underline{\RNInd}} 
% & \multicolumn{2}{c}{\underline{\RNDom}} 
% & \multicolumn{3}{c}{\underline{\Products}} 
% & \multirow{3}{*}{\textbf{Avg}}
% \\
% [0.5ex]
\textbf{Method}
& \multirow{2}{*}{\textbf{Retriever}}
& \multirow{2}{*}{\textbf{LM}}
% & \multicolumn{4}{c}{\underline{Self-BLEU-5 \lowerbetter}} 
% &
% & \multicolumn{4}{c}{\underline{Entity Entropy \higherbetter}} 
% &
& \multicolumn{4}{c}{\underline{\Mauve{} \higherbetter}} 
% &
& \multicolumn{4}{c}{\underline{Accuracy \higherbetter}} 
\\
[0.7ex]
\textit{(Dataset)}
& 
& 
% & \YelpNonSc % Self-BLEU
% & { }\AGNonSc % Self-BLEU
% & \IMDbNonSc % Self-BLEU
% & { }\SSTNonSc % Self-BLEU
% & 
% & { }\YelpNonSc % Entity Entropy
% & { }\AGNonSc % Entity Entropy 
% & \IMDbNonSc % Entity Entropy 
% & { }\SSTNonSc % Entity Entropy 
% & 
& \YelpNonSc % Mauve
& \AGNonSc % Mauve
& \IMDbNonSc % Mauve
& \SSTNonSc % Mauve
% & 
& \YelpNonSc % Accuracy
& \AGNonSc % Accuracy
& \IMDbNonSc % Accuracy
& \SSTNonSc % Accuracy
\\ 
\midrule
 \gold &  - & - 
 % & 27.5  &  17.1  & 27.9   &  35.5  
 % & 7.1   & 6.6   &  7.5  &  3.2 
 &  -  &  -  &  -  & -   
 & 94.5  & 90.8   & 91.3   & 88.2
 \vspace{0.75ex} \\ 
\toprule 
% \ZeroGen \ig{Ye2022ZeroGenEZ} & -  &  \GPTTwoXLShort 
% &  \noeval  &  \noeval  &  \norelease  &  \textbf{15.3}  
% &  \noeval  &  \noeval  &  \norelease  &  4.9  
% &  \noeval  &  \noeval  &  \norelease{}  &  \textbf{52.0}  
% &  \noeval{}  &  \noeval{}  &  \norelease{}  &  82.4
% \\
 % \ProGen \ig{ye-etal-2022-progen} & -  &  \GPTTwoXLShort 
 % &  \norelease  &  \norelease  &  \norelease  &  \norelease
 % &  \norelease  &  \norelease  &  \norelease  &  \norelease  
 % &  \norelease  &  \norelease  &  \norelease  &  \norelease
 % &  \norelease  &  \norelease  &  \norelease  &  \norelease
 % \\
 \SunGen \ig{gao2023selfguided} & -  &  \GPTTwoXLShort 
 % &  \norelease{}  &  \norelease{}  &  \textbf{15.4}  &  \norelease{}  
 % &  \norelease{}  &  \norelease{}  &  4.9  &  \norelease{}  
 &  \norelease{}  &  \norelease{}  &  68.7  &  \norelease{}  
 & \norelease{}  &  \norelease{}  &  84.9  &  \norelease{}
 \\
 \ReGen \ig{yu-etal-2023-regen} &  \BERT  & BERT 
 % &  \norelease{}  &  56.5  &  \norelease{}  &  \norelease{}  
 % &  \norelease{}  &  \textbf{8.1}  &  \norelease{}  &  \norelease{}  
 &  \norelease{}  &  68.1  &  \norelease{}  &  \norelease{}  
 &  \norelease{}  &  82.7  &  \norelease{}  & \norelease{}
 \\
 \LetsSynth \ig{wang-etal-2023-lets} & -  &  \GPTDavinciShortLower 
 % &  \noeval  &  \noeval  &  62.2  &  \noeval  
 % &  \noeval  &  \noeval  &  5.7  &  \noeval  
 &  \noeval  &  \noeval  &  62.0  &  \noeval  
 &  \noeval  &  \noeval  &  \textbf{87.1}  &  \noeval
 \\
 \AttrPromptShort \ig{yu2023large}  & - &  \ChatGPTShortLower 
 % &  70.3  &  39.8  &  \norelease  &  71.5  
 % &  3.4  &  6.0  &  \norelease  &  3.4  
 &  55.9  &  52.8  &  \norelease  &  50.0  
 &  89.3  &  79.8 & \norelease{}  &  80.8
 \\
 \toprule
\multicolumn{11}{c}{\underline{\textsc{Zero shot}}} \vspace{1ex} \\
 \oursword & \ContrieverShort &  \LLaMaShortNonSc 
 % &  70.2  &  29.3  &  66.3  &  41.9  
 % &  5.4  &  7.1  &  5.7  &  4.5  
 &  67.9  &  89.5  &  58.5  &  50.0  
 &  85.6  &  85.3  &  82.9  &  80.2
 \\
 \oursword & \ContrieverShort &  \ClaudeShortNonSc 
 % &  70.3  &  31.5  &  51.5  &  45.3  
 % &  \textbf{5.5}  &  6.6  &  5.3  &  \best{4.8}  
 &  54.0  &  94.2  &  55.9  &  50.0  
 &  87.5  &  85.6  &  83.6  &  82.5
 \\
%  [0.75ex]
%  \oursword & \BM &  \LLaMaShortNonSc 
% & 70.6  &  28.7  & 62.2   &  36.5  
%  & 4.7   & 7.0   &  5.6  &  5.1
%  & 64.7   &  90.3  &  60.5  & 50.0  
%  & 83.2  & 84.3   & 74.1   &  \best{84.4}
%  \\
%  \oursword & \BM &  \ClaudeShortNonSc 
%  & 72.9  &  30.9  & 50.4   &  36.9  
%  & 4.5   & 6.5   &  5.1  &  \best{5.4}
%  &  54.6  &  90.8  &  53.2  & 50.0  
%  & 86.7  & 84.2   & 79.1   & 82.6
%  \\
[0.75ex]
\multicolumn{11}{c}{\underline{\textsc{3-shot \RetrICL}}} \vspace{1ex} \\
 \oursword & \ContrieverShort &  \LLaMaShortNonSc 
 % &  59.5  &  34.2  &  62.9  &  26.3  
 % &  4.9  &  7.2  &  5.7  &  3.8  
 &  \textbf{84.9}  &  92.6  &  \textbf{72.6}  &  50.0  
 &  89.9  &  84.6  &  84.8  &  \textbf{83.8}
 \\
 \oursword & \ContrieverShort &  \ClaudeShortNonSc
 % &  \textbf{58.5}  &  \textbf{23.7}  &  38.0  &  \textbf{24.6} 
 % &  4.9  &  6.7  &  \textbf{5.9}  &  4.3 
 &  70.3  &  \textbf{95.8}  &  58.0  &  50.0  
 &  \textbf{91.3}  &  \textbf{86.0}  &  86.3  &  80.6
 \\
 % [0.75ex]
 % \oursword & \BM &  \LLaMaShortNonSc 
 % & 66.6  &  32.0  & 59.7   &  25.3  
 % & 5.1   & 7.2   &  5.6  &  4.8
 % &  81.9  &  92.5  &  \best{78.7}  & 50.0  
 % &  90.7 & 84.3   & 84.7  & \best{84.4}
 % \\
 % \oursword & \BM &  \ClaudeShortNonSc
 % & 59.9  &  24.6  & 41.9   &  26.8  
 % & 5.0   & 6.7   &  5.4  &  4.9 
 % &  63.3  &  \best{96.0}  &  58.5  & 50.0  
 % & 89.4  & 84.1   & 81.6  & 82.3
 % \\
\bottomrule
\end{tabular}
}
\vspace{-1ex}
\caption{
\Mauve{} and distillation accuracy on synthetic datasets released by prior work, subsampled to 6K examples as described in \autoref{sec:detailed-baseline-comparison}. For our method, we retrieve using Contriever, and generate 6K examples using teachers \LLaMaShortNonSc{} 13B Chat and \ClaudeShortNonSc{} Instant-v1.2. Accuracy reports the average of five \DistilBERT{} training runs using \citet{yu2023large}'s hyperparameters (\mbox{std.~dev.~$\le 2.0$} in all cases). Best results for each task are indicated in \textbf{bold}. Tasks not covered by prior work are marked {\noeval}; those evaluated without dataset release are marked {\norelease}. 
}
\vspace{-3ex}
\label{tab:baselines-combined-main}
\end{table}

==> table/baselines-intrinsic.tex <==
\begin{table*}[!h]
\centering
\sisetup{round-mode=places, round-precision=1} % Set the rounding precision
\setlength{\tabcolsep}{1.9pt}
\footnotesize{

\begin{tabular}{
C{1.65cm}  % Method
C{1.45cm}  % Teacher LM
C{1.35cm}  % Retriever
c % S[table-format=3.2]  % Yelp Self-BLEU
c % S[table-format=3.2]  % AG News Self-BLEU
c % S[table-format=3.2]  % IMDb Self-BLEU
c % S[table-format=3.2]  % SST-2 Self-BLEU
% c 
|c % S[table-format=3.2]  % Yelp Entity Entropy
c % S[table-format=3.2]  % AG News Entity Entropy
c % S[table-format=3.2]  % IMDb Entity Entropy
c  % S[table-format=3.2]  % SST-2 Entity Entropy
% c 
|c % S[table-format=3.2]  % Yelp Mauve
c % S[table-format=3.2]  % AG News Mauve
c % S[table-format=3.2]  % IMDb Mauve
c % S[table-format=3.2]  % SST-2 Mauve
}
\toprule
% \multirow{3}{*}{\textbf{Method}}
% & \multirow{3}{*}{ \textbf{Student LM} }
% & \multicolumn{1}{c}{\underline{\RNInd}} 
% & \multicolumn{2}{c}{\underline{\RNDom}} 
% & \multicolumn{3}{c}{\underline{\Products}} 
% & \multirow{3}{*}{\textbf{Avg}}
% \\
% [0.5ex]
\textbf{Method}
& \textbf{Teacher}
& \multirow{2}{*}{\textbf{Retriever}}
& \multicolumn{4}{c}{\underline{Self-BLEU-5 \lowerbetter}} 
% &
& \multicolumn{4}{c}{\underline{Entity Entropy \higherbetter}} 
% &
& \multicolumn{4}{c}{\underline{Mauve \higherbetter}} 
\\
[0.7ex]
\textit{(Dataset)}
& \textbf{LM}
& 
& \Yelp % Self-BLEU
& \AG % Self-BLEU
& \IMDb % Self-BLEU
& \SST{ } % Self-BLEU
% & 
& { }\Yelp % Entity Entropy
& \AG % Entity Entropy 
& \IMDb % Entity Entropy 
& \SST{ } % Entity Entropy 
% & 
& \Yelp % Mauve
& \AG % Mauve
& \IMDb % Mauve
& \SST % Mauve
\\ 
\midrule
 \gold &  - & - 
 & 27.5  &  17.1  & 27.9   &  35.5  
 & 7.1   & 6.6   &  7.5  &  3.2 
 &  -  &  -  &  -  & -   
 \vspace{0.75ex} \\ 
\toprule 
\ZeroGen \ig{Ye2022ZeroGenEZ}  &  \GPTTwoXL & - &  \noeval  &  \noeval  &  \norelease  &  \textbf{15.3}  &  \noeval  &  \noeval  &  \norelease  &  4.9  &  \noeval  &  \noeval  &  \norelease{}  &  \textbf{52.0}  \\
 \ProGen \ig{ye-etal-2022-progen}  &  \GPTTwoXL & - &  \norelease  &  \norelease  &  \norelease  &  \norelease
 &  \norelease  &  \norelease  &  \norelease  &  \norelease  &  \norelease  &  \norelease  &  \norelease  &  \norelease  \\
 \SunGen \ig{gao2023selfguided}  &  \GPTTwoXL & - &  \norelease{}  &  \norelease{}  &  \textbf{15.4}  &  \norelease{}  &  \norelease{}  &  \norelease{}  &  4.9  &  \norelease{}  &  \norelease{}  &  \norelease{}  &  68.7  &  \norelease{}  \\
 \ReGen \ig{yu-etal-2023-regen} & - &  \BERT  &  \norelease{}  &  56.5  &  \norelease{}  &  \norelease{}  &  \norelease{}  &  \textbf{8.1}  &  \norelease{}  &  \norelease{}  &  \norelease{}  &  68.1  &  \norelease{}  &  \norelease{}  \\
 \LetsSynth \ig{wang-etal-2023-lets}  &  \ChatGPTShort & - &  \noeval  &  \noeval  &  62.2  &  \noeval  &  \noeval  &  \noeval  &  5.7  &  \noeval  &  \noeval  &  \noeval  &  62.0  &  \noeval  \\
 \AttrPromptShort \ig{yu2023large}  &  \ChatGPTShort & - &  70.3  &  39.8  &  \norelease  &  71.5  &  3.4  &  6.0  &  \norelease  &  3.4  &  55.9  &  52.8  &  \norelease  &  50.0  \\
 \toprule
\multicolumn{15}{c}{\underline{\textsc{Zero shot}}} \vspace{1ex} \\
 \oursshort &  \LLaMa & \ContrieverShort &  70.2  &  29.3  &  66.3  &  41.9  &  5.4  &  7.1  &  5.7  &  4.5  &  67.9  &  89.5  &  58.5  &  50.0  \\
 \oursshort &  \Claude & \ContrieverShort &  70.3  &  31.5  &  51.5  &  45.3  &  \textbf{5.5}  &  6.6  &  5.3  &  4.8  &  54.0  &  94.2  &  55.9  &  50.0  \\
 [0.75ex]
 \oursshort &  \LLaMa & \BM 
& 70.6  &  28.7  & 62.2   &  36.5  
 & 4.7   & 7.0   &  5.6  &  5.1
 & 64.7   &  90.3  &  60.5  & 50.0   \\
 \oursshort &  \Claude & \BM 
 & 72.9  &  30.9  & 50.4   &  36.9  
 & 4.5   & 6.5   &  5.1  &  \best{5.4}
 &  54.6  &  90.8  &  53.2  & 50.0   \\
[0.75ex]
\multicolumn{15}{c}{\underline{\textsc{3-shot \RetrICL}}} \vspace{1ex} \\
 \oursshort &  \LLaMa & \ContrieverShort &  59.5  &  34.2  &  62.9  &  26.3  &  4.9  &  7.2  &  5.7  &  3.8  &  \textbf{84.9}  &  92.6  &  72.6  &  50.0  \\
 \oursshort &  \Claude & \ContrieverShort &  \textbf{58.5}  &  \textbf{23.7}  &  38.0  &  24.6  &  4.9  &  6.7  &  \textbf{5.9}  &  4.3  &  70.3  &  95.8  &  58.0  &  50.0  \\
 [0.75ex]
 \oursshort &  \LLaMa & \BM 
 & 66.6  &  32.0  & 59.7   &  25.3  
 & 5.1   & 7.2   &  5.6  &  4.8
 &  81.9  &  92.5  &  \best{78.7}  & 50.0   \\
 \oursshort &  \Claude & \BM 
 & 59.9  &  24.6  & 41.9   &  26.8  
 & 5.0   & 6.7   &  5.4  &  4.9 
 &  63.3  &  \best{96.0}  &  58.5  & 50.0   \\
\bottomrule
\end{tabular}
}
\vspace{-1ex}
\caption{
Intrinsic evaluations of synthetic datasets released by prior work. We subsample all to 6k examples before computing metrics as described in \S\ref{sec:expt-setup}. Within each dataset, we \textbf{bold} the best result. Tasks not evaluated by previous authors are denoted by {\noeval}, while those evaluated without dataset release are marked as {\norelease}. \ChatGPTShort{} is gpt-3.5-turbo.
}
\vspace{-2ex}
\label{tab:baselines-intrinsic}
\end{table*}

==> table/baselines-student.tex <==
\begin{table}[t!]
\centering
\sisetup{round-mode=places, round-precision=1} % Set the rounding precision
\setlength{\tabcolsep}{2pt}
\footnotesize{

\begin{tabular}{
C{1.6cm}  % Method
C{1.35cm}  % Teacher LM
C{0.7cm}  % Original dataset size
C{0.75cm} % S[table-format=3.2]  % Yelp Accuracy
C{0.75cm} % S[table-format=3.2]  % AG News Accuracy
C{0.75cm} % S[table-format=3.2]  % IMDb Accuracy
C{0.7cm} % S[table-format=3.2]  % SST-2 Accuracy
}
\toprule
% \multirow{3}{*}{\textbf{Method}}
% & \multirow{3}{*}{ \textbf{Student LM} }
% & \multicolumn{1}{c}{\underline{\RNInd}} 
% & \multicolumn{2}{c}{\underline{\RNDom}} 
% & \multicolumn{3}{c}{\underline{\Products}} 
% & \multirow{3}{*}{\textbf{Avg}}
% \\
% [0.5ex]
\textbf{Method}
& \textbf{Teacher / Retriever}
& \textbf{Data Size}
& \Yelp
& \AG
& \IMDb
& \SST
\\
\midrule
 \gold & -  & 6k  & 94.5  & 90.8   & 91.3   & 88.2   \\
\toprule
\ZeroGen \ig{Ye2022ZeroGenEZ}  &  \multirow{2}{*}{\GPTTwoXL}  & 6k  &  \noeval{}  &  \noeval{}  &  \norelease{}  &  82.4  \\
\textit{(Reported)}  &   &  200k  &  \noeval{}  &  \noeval{}  &  \textit{84.3}  &  \textit{87.3}  \\
[1.5ex]
\ProGen \ig{ye-etal-2022-progen}  &  \multirow{2}{*}{\GPTTwoXL}  & 6k  &  \norelease{}  &  \norelease{}  &  \norelease{}  &  \norelease{}  \\
\textit{(Reported)}  &   &  100k  &  \textit{89.4}  &  \textit{80.8}  &  \textit{84.1}  &  \textit{87.2}  \\
[1.5ex]
\SunGen \ig{gao2023selfguided}  &  \multirow{2}{*}{\GPTTwoXL}  & 6k  &  \norelease{}  &  \norelease{}  &  84.9  &  \norelease{}  \\
\textit{(Reported)}  &   &  200k  &  \textit{89.2}  &  \textit{80.5}  &  \textit{89.4}  &  \textit{89.5}  \\
[1.5ex]
\ReGen \ig{yu-etal-2023-regen}  &  \multirow{2}{*}{\BERT}  & 6k  &  \norelease{}  &  82.7  &  \norelease{}  & \norelease{}  \\
\textit{(Reported)}  &   &  20k  &  \textit{89.0}  &  \textit{85.0}  &  \textit{87.8}  &  \textit{85.3}  \\
[1.5ex]
\LetsSynth \ig{wang-etal-2023-lets}  &  \multirow{2}{*}{\ChatGPTShort}  & 6k  &  \noeval{}  &  \noeval{}  &  \textbf{87.1}  &  \noeval{}  \\
\textit{(Reported)}  &   &  21.2k  &  \noeval{}  &  \noeval{}  &  \textit{89.0}  &  \noeval{}  \\
[1.5ex]
\AttrPromptShort \ig{yu2023large}  &  \multirow{2}{*}{\ChatGPTShort}  & 6k  &  89.3  &  79.8 & \norelease{}  &  80.8  \\
\textit{(Reported)}  &   &  6k  &  \textit{90.6}  &  \textit{82.7}  &  \textit{85.9}  &  \textit{83.6}  \\
\toprule
\multicolumn{7}{c}{\underline{\textsc{Zero shot}}} \vspace{1ex} \\
 \oursshort  &  \LLaMa{} $+$ \ContrieverShort{} &  6k  &  85.6  &  85.3  &  82.9  &  80.2  \\
 [1.0ex]
 \oursshort  &  \Claude{} $+$ \ContrieverShort{} &  6k  &  87.5  &  85.6  &  83.6  &  82.5  \\
 [1.5ex]
 \oursshort  &  \LLaMa{} $+$ \BM{} &  6k  & 83.2  & 84.3   & 74.1   &  \best{84.4}  \\
 [1.0ex]
 \oursshort  &  \Claude{} $+$ \BM{} &  6k  & 86.7  & 84.2   & 79.1   & 82.6   \\
[1.5ex]
\multicolumn{7}{c}{\underline{\textsc{3-shot \RetrICL}}} \vspace{1ex} \\
 \oursshort  &  \LLaMa{} $+$ \ContrieverShort{}  &  6k  &  89.9  &  84.6  &  84.8  &  83.8  \\
 [1.0ex]
 \oursshort  &  \Claude{} $+$ \ContrieverShort{} &  6k  &  \textbf{91.3}  &  \textbf{86.0}  &  86.3  &  80.6  \\
 [1.5ex]
 \oursshort  &  \LLaMa{} $+$ \BM{}  &  6k  &  90.7 & 84.3   & 84.7  & \best{84.4}  \\
 [1.0ex]
 \oursshort  &  \Claude{} $+$ \BM{}  &  6k  & 89.4  & 84.1   & 81.6  & 82.3  \\
\bottomrule
\end{tabular}
}
\vspace{-1ex}
\caption{
Test accuracy of \ours{} \RetrICL{} against baselines after fine-tuning a \DistilBERT{} student. For each released dataset, we subsample to 6k examples to make a fair comparison. We train 5 student models and report the mean accuracy (std.~dev.~was $\le 2.0$ in all cases, thus we avoid reporting it for brevity). We report the \DistilBERT{} accuracy from the original paper (if available) in \textit{italics}. For each dataset, we \textbf{bold} the best result from the fair evaluation. Tasks not evaluated by previous authors are denoted by {\noeval}, while those evaluated without dataset release are marked as {\norelease}. \ChatGPTShort{} is gpt-3.5-turbo.
}
\vspace{-3ex}
\label{tab:baselines-student}
\end{table}

==> table/prompts.tex <==
% \begin{prompt}[title={Prompt \thetcbcounter: task-inversion prompt examples}, label=prompt:task-inversion-ex]
% \promptsection{Task 1. Political Bias detection}
% \\ 
% \promptsubsection{\fewgen} \prompttext{Write a single news article using \param{{label}}.
% \\ News Article: } \\ 
% \promptsubsection{\ours} \prompttext{News Article: \param{{article_retr[k]}}
% \\ Rewrite the above news article using \param{{label}}. 
% \\ Rewritten Article: }
% \\
% \promptsubsection{Verbalization} 
% \verbal{true}{harsh political language, using a mocking tone and toxic commentary};
% \verbal{false}{neutral language, using a reasonable tone and politically correct commentary} 
% \vspace{-1ex}
% \promptsection{Task 2. Humor detection in product questions}
% \\ 
% \promptsubsection{\fewgen} \prompttext{Write a short \param{{label}} question about \text{a} product on Amazon. Only include the question.
% \\ Product Question: }
% \\ 
% \promptsubsection{\ours} \prompttext{Product details: \param{{product_retr[k]}}
% \\ Write a short \param{{label}} question about the above product on Amazon. Only include the question.
% \\ Product Question: }
% \\
% \promptsubsection{Verbalization} 
% \verbal{non_humorous}{solemn};
% \verbal{humorous}{humorous}
% \end{prompt}

\begin{figure}[!th]
\includegraphics[width=0.48\textwidth]{figure/prompts-12Feb2024.png}

% \vspace{-1ex}
% \subfigure[AG News]{
%     \includegraphics[width=0.47\linewidth]{figure/entity-entropy-14Jan2024.png}
%     \label{fig:encoder_topic}
% } \hspace{-1ex} %\hfill

% \vspace{-1.5ex}
\centering
\caption{
Comparison: task inversion prompting to synthesize political news and humorous product questions.
}
\vspace{-1.5ex}
\label{fig:prompts}
\end{figure}


==> table/student.tex <==
\begin{table*}[!h]
\centering
\setlength{\tabcolsep}{3pt}
\tiny{
\begin{tabular}{
L{1.7cm}
L{2.4cm}  % Student
cc  % Realnews
c  % ToI
% p{0.1em}
c
c
c
c
}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multirow{2}{*}{ \textbf{Student LM} }
& \multicolumn{1}{c}{\underline{\TimesOfIndia}} 
& \multicolumn{2}{c}{\underline{\RealNewsDominant}} 
& \multicolumn{3}{c}{\underline{\AmazonProducts}} 
& \multirow{2}{*}{\textbf{Average}}
\\
[0.5ex]
&                      
& \ToITopics{} ($8$K) 
& \AGNews{} ($8$K)  
& \Hyper{} ($4$K)   
& \Category{} ($8$K) 
& \Humor{} ($2$K)   
& \Polarity{} ($4$K) 
&
\\ 
% &                               &         &         &         &         &         &  \\ 
% \cmidrule{1-2}                        \cmidrule{3-5} \cmidrule{7-9}
[-0.5ex]
\midrule
\multirow{3}{*}{\gold}          
& \TinyBERT{}                   &     77.83 &         87.9 &       81.23 &         70.41 &      89.22 &         87.09 & 82.28 \\
& \DistilBERT{}                 &     82.16 &        90.45 &       88.92 &         78.44 &      91.69 &         90.78 & 87.07 \\
& \DeBERTa{}                    &     83.97 &        91.02 &       93.23 &         81.52 &      93.06 &         95.26 & 89.68 \\

\midrule
\midrule

\multirow{3}{*}{\parbox{1.6cm}{\fewgen{} \hspace{3ex} \mbox{(0-shot)}}} 
& \TinyBERT{} (w. \Cart)        &  \text{56.94} (\best{71.96}) &  \text{66.29} (\decr{62.69}) &  \text{58.77} (\decr{57.85}) &    \text{51.1} (\decr{48.0}) &  \text{64.82} (\best{83.15}) &  \text{76.36} (\decr{74.55}) & 62.38 (66.37) \\
& \DistilBERT{} (w. \Cart)      &  \text{65.57} (\decr{59.45}) &  \text{69.74} (\decr{66.56}) &  \best{62.77} (\decr{58.77}) &  \text{59.52} (\decr{57.79}) &  \text{67.25} (\incr{67.74}) &  \text{78.96} (\incr{80.37}) & 67.30 (65.11) \\
& \DeBERTa{} (w. \Cart) &  \text{58.88} (\decr{49.82}) &  \text{70.39} (\decr{64.45}) &  \text{70.15} (\incr{70.46}) &  \text{58.73} (\decr{57.25}) &  \text{72.17} (\decr{70.31}) &  \text{81.12} (\incr{87.69}) & 68.57 (66.66) \\
% [1ex] 

\midrule

\multirow{3}{*}{\parbox{2cm}{\ours{} \mbox{(0-shot)}}}
& \TinyBERT{} (w. \Cart)        &  \text{66.77} (\incr{68.56}) &  \text{80.72} (\best{84.06}) &  \best{64.31} (\decr{58.15}) &   \text{57.88} (\best{61.5}) &  \text{75.89} (\incr{78.15}) &  \best{80.08} (\decr{79.45}) & 70.94 (\best{71.64}) \\
& \DistilBERT{} (w. \Cart)      &  \text{72.71} (\best{72.86}) &  \text{84.24} (\best{85.54}) &   \text{61.23} (\decr{60.0}) &  \text{65.69} (\best{70.97}) &  \best{84.63} (\decr{79.91}) &  \best{82.18} (\decr{79.71}) & \best{75.11} (74.83) \\
& \DeBERTa{} (w. \Cart) &  \best{74.22} (\decr{73.95}) &  \text{84.76} (\best{85.55}) &  \best{71.69} (\decr{70.15}) &  \text{69.42} (\best{70.12}) &  \text{82.36} (\best{85.71}) &  \best{88.63} (\decr{88.02}) & 78.51 (\best{78.92}) \\

\midrule
\midrule

\multirow{2}{*}{\textbf{Method}}
& \multirow{2}{*}{ \textbf{Student LM} }
& \multicolumn{1}{c}{\underline{\TimesOfIndia}} 
& \multicolumn{2}{c}{\underline{\RealNewsDominant}} 
& \multicolumn{3}{c}{\underline{\AmazonProducts}} 
& \multirow{2}{*}{\textbf{Average}}
\\
[0.5ex]
&                      
& \ToITopics{} ($8$K) 
& \AGNews{} ($8$K)  
& \Hyper{} ($4$K)   
& \Category{} ($8$K) 
& \Humor{} ($2$K)   
& \Polarity{} ($4$K)
&
\\ 
[-0.5ex]
\midrule

\multirow{3}{*}{\parbox{1.6cm}{\fewgen{} \hspace{3ex} \mbox{(32-shot)}}}  
& \TinyBERT{} (w. \Cart)        &  \best{72.68} (\decr{72.05}) &  \text{82.94} (\incr{83.22}) &  \text{63.08} (\incr{65.85}) &  \text{58.14} (\decr{46.08}) &  \best{83.19} (\decr{83.18}) &   \text{80.29} (\decr{77.2}) & 73.39 (71.26) \\
& \DistilBERT{} (w. \Cart)      &  \best{76.83} (\decr{58.66}) &  \text{85.22} (\incr{85.32}) &  \text{64.62} (\best{69.54}) &   \text{67.7} (\decr{51.88}) &  \text{85.57} (\decr{84.64}) &  \text{84.29} (\decr{79.04}) & 77.37 (71.51) \\
& \DeBERTa{} (w. \Cart) &  \best{78.54} (\decr{75.87}) &  \text{85.95} (\decr{84.51}) &  \text{75.69} (\decr{74.46}) &   \text{66.47} (\decr{34.7}) &  \text{88.62} (\incr{88.96}) &   \text{89.5} (\best{90.72}) & 80.80 (74.87) \\
% [1ex] 
\midrule

\multirow{3}{*}{\parbox{2cm}{\ours{} \mbox{(3-shot \textsc{Retr})}}} 
& \TinyBERT{} (w. \Cart)        &  \text{70.78} (\incr{71.94}) &  \text{81.67} (\decr{81.33}) &  \text{64.62} (\decr{61.85}) &  \text{59.55} (\incr{61.87}) &  \text{81.31} (\incr{82.93}) &   \best{81.23} (\decr{80.7}) & 73.19 (73.44) \\
& \DistilBERT{} (w. \Cart)      &  \text{74.91} (\incr{75.18}) &  \text{83.28} (\incr{84.24}) &  \text{64.92} (\decr{61.54}) &  \text{67.07} (\best{70.83}) &  \best{86.01} (\decr{84.47}) &  \best{84.89} (\decr{84.25}) & 76.85 (\best{76.75}) \\
& \DeBERTa{} (w. \Cart) &  \text{76.42} (\incr{77.42}) &  \text{84.83} (\incr{85.59}) &   \text{76.0} (\best{77.23}) &  \text{70.55} (\best{73.57}) &  \best{90.18} (\decr{88.72}) &   \text{84.45} (\incr{89.7}) & 80.40 (\best{82.04}) \\
[1ex] % \midrule

\multirow{3}{*}{\parbox{2cm}{\ours{} \mbox{(32-shot \textsc{No-Retr})}}} 
& \TinyBERT{} (w. \Cart)        &  \text{70.03} (\incr{71.11}) &  \text{80.89} (\best{83.41}) &  \text{65.85} (\best{67.08}) &  \text{63.59} (\best{63.94}) &  \text{81.81} (\decr{77.62}) &  \text{79.52} (\decr{79.12}) & 73.61 (\best{73.71}) \\
& \DistilBERT{} (w. \Cart)      &  \text{73.42} (\incr{74.57}) &  \text{84.61} (\best{85.89}) &  \text{64.62} (\decr{62.77}) &  \text{70.35} (\incr{70.67}) &  \text{84.81} (\decr{80.22}) &  \text{82.11} (\decr{81.08}) & 76.65 (75.87) \\
& \DeBERTa{} (w. \Cart) &  \text{74.09} (\incr{76.16}) &  \text{84.39} (\best{87.08}) &   \text{74.46} (\incr{76.0}) &  \text{71.71} (\incr{72.68}) &  \text{87.45} (\incr{87.61}) &   \text{87.9} (\decr{86.12}) & 80.00 (80.94) \\
                                
\bottomrule
\end{tabular}
}
\vspace{-1ex}
\caption{
Test Accuracy ($\uparrow$) after distilling a student LM from LLaMa-2 Chat 13B. We report mean of 5 runs. Filtering based on training dynamics (w. \Cart) is done by keeping top-83\% of most ambiguous examples from a \DistilBERT{} training run. The top half considers zero-shot synthesis and bottom half uses in-context learning.
}
\vspace{-3ex}
\label{tab:student}
\end{table*}




% \begin{table*}[t!]
% % \vspace{-0.5em}
% \centering
% \footnotesize{
% \begin{tabular}{lcccc}
% \toprule 
% \bf Dataset & \bf Task  & \bf Class  & \bf \# Test & \bf Metric  \\ \midrule
% Youtube & Spam & & &  & 74.4\% & 91.7\%\\ %\hline
% AGNews & News Topic &4  & 7.6k & Accuracy \\ %\hline
% DBPedia & Wikipedia Topic & 14 & 70k & Accuracy  \\
% Yahoo Topics & Web QA Topic & 10 & 60k & Accuracy  \\
% NYT & News Topic & 9 & 30k & F1  \\\hline
% IMDB & Movie Review Sentiment &2  & 25k & Accuracy  \\ %\hline
% MR & Movie Review Sentiment& 2& 2k & Accuracy  \\ %\hline
% SST-2 & Movie Review Sentiment& 2 & 0.8k & Accuracy \\ %\hline
% Amazon & Product Review Sentiment& 2 & 40k & Accuracy \\ %\hline
% Yelp &Restaurant Review Sentiment& 2 & 38k & Accuracy \\ %\hline
%             \bottomrule
% \end{tabular}

% \vspace{-1ex}
% }
% \caption{
% Student distillation performance.
% }
% \vspace{-1.5ex}
% \label{tab:student}
% \end{table*}


% \begin{table}[t]
% \centering
% 	\resizebox{\columnwidth}{!}{
% 		\begin{tabular}{ccccc}
			% \toprule \bf Dataset & \bf Task  & \bf Class  & \bf \# Test & \bf Metric  \\ \midrule
			% %Youtube &Spam& & &  & 74.4\% & 91.7\%\\ %\hline
   %          AGNews & News Topic &4  & 7.6k & Accuracy \\ %\hline
   %          DBPedia & Wikipedia Topic & 14 & 70k & Accuracy  \\
   %          Yahoo Topics & Web QA Topic & 10 & 60k & Accuracy  \\
   %          NYT & News Topic & 9 & 30k & F1  \\\hline
   %          IMDB & Movie Review Sentiment &2  & 25k & Accuracy  \\ %\hline
   %          MR & Movie Review Sentiment& 2& 2k & Accuracy  \\ %\hline
   %          SST-2 & Movie Review Sentiment& 2 & 0.8k & Accuracy \\ %\hline
   %          Amazon & Product Review Sentiment& 2 & 40k & Accuracy \\ %\hline
   %          Yelp &Restaurant Review Sentiment& 2 & 38k & Accuracy \\ %\hline
   %          \bottomrule
% 		\end{tabular}
% 	}
% 	\caption{Dataset statistics. }
% 	\label{tab:dataset}
%\lgspace
% \end{table}


% \begin{table*}[!t]
% % \resizebox{\linewidth}{!}{%
% % \scalebox{0.57}{
% \vspace{-0.3ex}
% \centering 
% \renewcommand\arraystretch{0.9}
% \fontsize{7.5}{9.5}\selectfont \setlength{\tabcolsep}{0.5em}
% \resizebox{0.99\linewidth}{!}{%
% \begin{tabular}{l|ccccc|cccccc|c}
% \toprule
% \bf    Task ($\rightarrow$)     & \multicolumn{5}{c|}{\bf{Topic Classification}}  &  \multicolumn{6}{c|}{\bf{Sentiment Classification}} & \bf All  \\  \hline   
% \bf    Method ($\downarrow$) / Dataset ($\rightarrow$)    & \bf  AG News & \bf DBPedia & \bf Yahoo  & \bf NYT & \multicolumn{1}{>{\columncolor{maroon}}c}{\bf Avg.} & \bf  IMDB & \bf MR & \bf SST-2 & \bf Amazon  & \bf Yelp &  \multicolumn{1}{>{\columncolor{lightblue}}c}{\bf Avg.} & \multicolumn{1}{>{\columncolor{yellow}}c}{\bf Avg.} \\ \hline
% \multicolumn{10}{l}{\emph{Zero-shot Learning via Direct Inferencing on Test Data}}  \\\hline 
% % Dataless~\shortcite{dataless} & 69.6 & 63.4 & 40.4 & 44.2	& \multicolumn{1}{>{\columncolor{maroon}}c}{59.4} & 50.5 & 55.2 & 52.2 & 52.8 &  51.1 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{52.4} & \multicolumn{1}{>{\columncolor{yellow}}c}{55.9}	\\
% NSP-BERT~\shortcite{sun2021nsp} & 78.1 & 69.4 & 47.0 & 54.6 & \multicolumn{1}{>{\columncolor{maroon}}c}{ 62.3} & 73.1 & 74.4 & 75.6 & 69.4 & 66.3 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{71.8}& \multicolumn{1}{>{\columncolor{yellow}}c}{67.5} \\ 
% % Prompt~\shortcite{van2022don} & 34.0 & 36.4 & 28.2 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---}  & 78.4 & 71.1 & 77.4 & 81.5  & 81.9 & \multicolumn{1}{>{\columncolor{lightblue}}c}{78.0}  & \multicolumn{1}{>{\columncolor{yellow}}c}{---}  \\
% Prompt~\shortcite{schick-schutze-2021-exploiting} & 73.2 & 71.3 & 44.1 & 57.4 & \multicolumn{1}{>{\columncolor{maroon}}c}{61.5}  &  74.8 & 73.2 & 75.9 & 80.2 & 78.1 & \multicolumn{1}{>{\columncolor{lightblue}}c}{76.4}  & \multicolumn{1}{>{\columncolor{yellow}}c}{68.9}  \\
% KNN-Prompt~\shortcite{shi2022nearest} & 78.8 & --- & 51.0 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---}  &  --- & 78.2 & 84.2 & 85.7 & --- & \multicolumn{1}{>{\columncolor{lightblue}}c}{---} & \multicolumn{1}{>{\columncolor{yellow}}c}{---} \\
% GPT-3$^\ddagger$~\shortcite{zhao2021calibrate} & 73.9 & 59.7 & 54.7 & 57.0 & \multicolumn{1}{>{\columncolor{maroon}}c}{61.3}  & 75.8 & 76.3 & 87.2 & 75.0 & 78.5 & \multicolumn{1}{>{\columncolor{lightblue}}c}{78.6} & \multicolumn{1}{>{\columncolor{yellow}}c}{69.9} \\
% \hline
% \multicolumn{10}{l}{\emph{Zero-shot Learning via Generating Task-specific Datasets}} 
%  \\\hline
% % LOTClass$^{\natural}$~(\emph{Our ReImp.}) & 82.3\std{1.0}& 77.8\std{2.1} & 52.6\std{1.4} & 55.1\std{2.0} &  \multicolumn{1}{>{\columncolor{maroon}}c}{66.9}  & 73.4\std{2.0} & 72.6\std{1.8} & 75.3\std{0.9} & 77.9\std{1.2} & 74.8\std{1.3}&\multicolumn{1}{>{\columncolor{lightblue}}c}{74.8} & \multicolumn{1}{>{\columncolor{yellow}}c}{71.9}\\
% SuperGen$^\ddagger$~\shortcite{meng2022generating} & 77.4\std{1.5} & 66.5\std{2.0} & 40.8\std{1.5}& 53.9\std{1.5} & \multicolumn{1}{>{\columncolor{maroon}}c}{59.7} & 85.8\std{1.6} & 81.9\std{0.9} & 88.6\std{0.5} & 91.0\std{0.9} & \bf  93.6\std{0.6} &  \multicolumn{1}{>{\columncolor{lightblue}}c}{88.1} & \multicolumn{1}{>{\columncolor{yellow}}c}{73.9}
% \\
% Mining$^*$~\shortcite{van2022don} & 79.2 & 80.4 & 56.1 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---} & 86.7 & 80.5 & 85.6 & 92.0 & 92.0 & \multicolumn{1}{>{\columncolor{lightblue}}c}{87.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{---}\\
% Mining$^{*\natural}$ (\emph{Our ReImp.}) & 79.7\std{1.0} & 82.1\std{0.6} & 57.0\std{0.6} & 68.6\std{0.9} & \multicolumn{1}{>{\columncolor{maroon}}c}{71.9}  &
% 87.1\std{0.6}  & 79.9\std{0.7} &  85.0\std{0.6} & 92.1\std{0.5} & 92.3\std{0.5} & \multicolumn{1}{>{\columncolor{lightblue}}c}{87.2} & \multicolumn{1}{>{\columncolor{yellow}}c}{79.6}\\
% % \hline
% \bf {\ours}  (Our Method) & \bf{85.0\std{0.8}} & \bf 87.6\std{0.9}& \bf  59.4\std{0.8} & \bf  74.5\std{1.1} & \multicolumn{1}{>{\columncolor{maroon}}c}{\bf 76.6}  & \bf  89.9\std{0.5} & \bf  82.5\std{0.7} & \bf  88.9\std{0.4} & \bf  92.3\std{0.4} &  93.0\std{0.5} & \multicolumn{1}{>{\columncolor{lightblue}}c}{\bf 89.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{\bf 83.0}\\
% \hline
% % \hline
% % $\tx{}^{\sharp}$
% % \midrule
% %% *********************************************************************
% \multicolumn{10}{l}{\emph{\bf{For Reference Only}: Using labeled data from other tasks / task-specific corpus / external knowledge base.}}  
% \\ \hline
% TE-NLI (Best)$^\dagger$~\shortcite{yin-etal-2019-benchmarking} & 78.0 & 73.0 & 43.8 & 70.7 & \multicolumn{1}{>{\columncolor{maroon}}c}{66.4}  & 64.6 & 68.3  & 68.6 & 76.7 & 73.5 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{70.3} & \multicolumn{1}{>{\columncolor{yellow}}c}{68.6} \\
% NLI-ST $^{\dagger\sharp}$~\shortcite{gera2022zero} & 76.5 & 92.2 & 59.8 & --- & \multicolumn{1}{>{\columncolor{maroon}}c}{---}  & 92.5 & --- & --- & 94.3 & --- &  \multicolumn{1}{>{\columncolor{lightblue}}c}{---} & \multicolumn{1}{>{\columncolor{yellow}}c}{---} \\
% % NATCAT$^\dagger$~\shortcite{chu2021natcat} & 68.8 &  81.9 & 57.8 & 42.0 & \multicolumn{1}{>{\columncolor{maroon}}c}{62.6}  & 54.0 & 51.0 & 65.0 & 66.8 & 75.2 &  \multicolumn{1}{>{\columncolor{lightblue}}c}{62.4} & \multicolumn{1}{>{\columncolor{yellow}}c}{62.5}\\
% KPT$^{\sharp,\S}$~\shortcite{hu-etal-2022-knowledgeable} & 84.8 & 82.2  & 61.6 & 72.1 &\multicolumn{1}{>{\columncolor{maroon}}c}{75.2}  & 91.2 & --- & --- & 92.8 & --- &  \multicolumn{1}{>{\columncolor{lightblue}}c}{---} & \multicolumn{1}{>{\columncolor{yellow}}c}{---} \\
% LOTClass$^\sharp$~\shortcite{meng-etal-2020-text} & 86.2 & 91.1 & 55.7 & 49.5 & \multicolumn{1}{>{\columncolor{maroon}}c}{70.7}  & 86.5 & 70.8 & 80.9 & 91.7 & 87.6 & \multicolumn{1}{>{\columncolor{lightblue}}c}{83.5} & \multicolumn{1}{>{\columncolor{yellow}}c}{77.1} \\
% X-Class$^\sharp$~\shortcite{wang-etal-2021-x} & 85.7 & 91.3 & 50.5 & 68.5 & \multicolumn{1}{>{\columncolor{maroon}}c}{74.0}  & 89.0 & 78.8 & 84.8 & 90.4 & 90.0 & \multicolumn{1}{>{\columncolor{lightblue}}c}{86.5} & \multicolumn{1}{>{\columncolor{yellow}}c}{80.3} \\
% %  \midrule
% \bottomrule
% \end{tabular}
% }
% \vspace{-1ex}
% \caption{Main results. We report average performance and standard deviation across 5 runs \emph{if fine-tuning is applied}. $*$: concurrent work, $\natural$: use the same corpus and template as {\ours} for \emph{fair comparisons}, $\dagger$: use labeled data from auxiliary tasks, $\sharp$: use task-specific corpus,  $\ddagger$: use billion-scale PLMs, $\S$: use additional knowledge base.}
% \label{tab:main_f1}
% % }
% \vspace{-1ex}
% \end{table*}


